A Defect is Being Born: How Close Are We? A Time Sensitive Forecasting Approach

Background. Defect prediction has been a highly active topic among researchers in the Empirical Software Engineering field. Previous literature has successfully achieved the most accurate prediction of an incoming fault and identified the features and anomalies that precede it through just-in-time prediction. As software systems evolve continuously, there is a growing need for time-sensitive methods capable of forecasting defects before they manifest. Aim. Our study seeks to explore the effectiveness of time-sensitive techniques for defect forecasting. Moreover, we aim to investigate the early indicators that precede the occurrence of a defect. Method. We will train multiple time-sensitive forecasting techniques to forecast the future bug density of a software project, as well as identify the early symptoms preceding the occurrence of a defect. Expected results. Our expected results are translated into empirical evidence on the effectiveness of our approach for early estimation of bug proneness.

==> RevisionsEnvs.tex <==
% =========================================
% Reviewer Color Configuration
% =========================================

% Toggle to enable/disable reviewer colors
\newif\ifshowReviewColors
% \showReviewColorstrue   % set to 
\showReviewColorsfalse 
% to disable colors

% Define reviewer colors
\usepackage[table]{xcolor} % "table" option recommended
\usepackage{colortbl}      % for \arrayrulecolor

\definecolor{ReviewerAColor}{RGB}{0,128,128} % teal
\definecolor{ReviewerBColor}{RGB}{200,0,200} % magenta
\definecolor{ReviewerCColor}{RGB}{220,0,0}   % red

% =========================================
% Inline reviewer commands
% =========================================

\newcommand{\ReviewerA}[1]{%
  \ifshowReviewColors
    \textcolor{ReviewerAColor}{#1}%
  \else
    \textcolor{black}{#1}%
  \fi
}

\newcommand{\ReviewerB}[1]{%
  \ifshowReviewColors
    \textcolor{ReviewerBColor}{#1}%
  \else
    \textcolor{black}{#1}%
  \fi
}

\newcommand{\ReviewerC}[1]{%
  \ifshowReviewColors
    \textcolor{ReviewerCColor}{#1}%
  \else
    \textcolor{black}{#1}%
  \fi
}

% =========================================
% Block environments (text + tables auto-colored)
% =========================================

\newenvironment{ReviewerAEnv}
  {%
    \begingroup
    \ifshowReviewColors
      \color{ReviewerAColor}%
      \arrayrulecolor{ReviewerAColor}% table borders in same color
    \else
      \color{black}%
      \arrayrulecolor{black}%
    \fi
  }
  {%
    \arrayrulecolor{black}% restore default for following tables
    \endgroup
  }

\newenvironment{ReviewerBEnv}
  {%
    \begingroup
    \ifshowReviewColors
      \color{ReviewerBColor}%
      \arrayrulecolor{ReviewerBColor}%
    \else
      \color{black}%
      \arrayrulecolor{black}%
    \fi
  }
  {%
    \arrayrulecolor{black}%
    \endgroup
  }

\newenvironment{ReviewerCEnv}
  {%
    \begingroup
    \ifshowReviewColors
      \color{ReviewerCColor}%
      \arrayrulecolor{ReviewerCColor}%
    \else
      \color{black}%
      \arrayrulecolor{black}%
    \fi
  }
  {%
    \arrayrulecolor{black}%
    \endgroup
  }

==> preamble.tex <==
% -----------------------------------------------------------------------------
% IEEE Setup
% -----------------------------------------------------------------------------
\IEEEoverridecommandlockouts

% -----------------------------------------------------------------------------
% Core Packages
% -----------------------------------------------------------------------------
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{float}
\usepackage{color}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{todonotes}
\usepackage{hyperref}
\usepackage{xurl}
\usepackage{balance}
\usepackage{flushend}
% \usepackage{biblatex}
% -----------------------------------------------------------------------------
% Font & Symbols
% -----------------------------------------------------------------------------
\RequirePackage{fontawesome}


% -----------------------------------------------------------------------------
% Custom Colors
% -----------------------------------------------------------------------------
\definecolor{gray05}{gray}{.95}
\definecolor{gray10}{gray}{.9}
\definecolor{gray20}{gray}{.8}
\definecolor{gray30}{gray}{.7}
\definecolor{gray40}{gray}{.6}
\definecolor{gray50}{gray}{.5}
\definecolor{arsenic}{rgb}{0.23, 0.27, 0.29}

\usepackage[many,breakable]{tcolorbox}

% Define colors for use in tcolorbox
\definecolor{main}{HTML}{CFCFCF}  % Main background color
\definecolor{sub}{HTML}{CFCFCF}   % Sub background color

% Global settings for tcolorbox
\tcbset{
    sharp corners,           % Box with sharp corners
    colback = white,         % Background color
    before skip = 0.2cm,     % Space before the box
    after skip = 0.5cm       % Space after the box
}

% Define a custom tcolorbox style
\newtcolorbox{boxC}{
    colback = sub,  % Background color
    boxrule = 0pt   % No border
}

% Custom environment for key takeaways
\newcounter{keyTakeAwaysCounter} % Counter for key takeaways
\setcounter{keyTakeAwaysCounter}{0} % Initialize counter

\newenvironment{keyTakeAways}[1][Key Take Away]{
    \addtocounter{keyTakeAwaysCounter}{1} % Increment counter
    \begin{boxC}
    \faLightbulbO ~ \thekeyTakeAwaysCounter. \textbf{#1}.\\
}{
    \end{boxC}
}


\newcounter{keyRQAnswerCounter}
\setcounter{keyRQAnswerCounter}{0}

\newenvironment{keyRQAnswer}[1][RQAnswer]
    {
        \addtocounter{keyRQAnswerCounter}{1}
        \begin{boxC}{\faKey ~ \thekeyRQAnswerCounter. #1}
    }{
     \end{boxC}
    }
% Re-definition of BibTeX command for the logo
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


\renewcommand{\arraystretch}{1.4}

% -----------------------------------------------------------------------------
% Bibliography Setup
% -----------------------------------------------------------------------------
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}
\usepackage{cite}


% % Custom LaTeX commands for marking reviewer changes
% \newcommand{\ReviewerA}[1]{\textcolor{teal}{#1}}  % teal Changes for Reviewer A
% \newcommand{\ReviewerB}[1]{\textcolor{magenta}{#1}}   % magenta Changes for Reviewer B
% \newcommand{\ReviewerC}[1]{\textcolor{red}{#1}} % blue Changes for Reviewer C

% \newenvironment{ReviewerAEnv}
%   {\color{teal}} % begin
%   {}             % end

% \newenvironment{ReviewerBEnv}
%   {\color{magenta}}
%   {}

% \newenvironment{ReviewerCEnv}
%   {\color{red}}
%   {}

% \newenvironment{ReviewerMinorEnv}
%   {\color{black}}
%   {}



\input{RevisionsEnvs}
